Estimating optimal PAC-Bayes bounds with Hamiltonian Monte Carlo

An important yet underexplored question in the PAC-Bayes literature is how much tightness we lose by restricting the posterior family to factorized Gaussian distributions when optimizing a PAC-Bayes bound. We investigate this issue by estimating data-independent PAC-Bayes bounds using the optimal posteriors, comparing them to bounds obtained using MFVI. Concretely, we (1) sample from the optimal Gibbs posterior using Hamiltonian Monte Carlo, (2) estimate its KL divergence from the prior with thermodynamic integration, and (3) propose three methods to obtain high-probability bounds under different assumptions. Our experiments on the MNIST dataset reveal significant tightness gaps, as much as 5-6\% in some cases.

==> ce_rc_table_old.tex <==
\begin{table}[h!]
\caption{Training and test metrics and RC estimates using our three bounds, in terms of the cross-entropy loss. \textbf{Bold} numbers indicate the tighter certificate out of the Gibbs and MFVI ones for the same dataset. }
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}|lll|lll|ll|ll|@{}}
\toprule
\multicolumn{3}{|l|}{Setup}            & \multicolumn{3}{l|}{Train/test stats} & \multicolumn{2}{l|}{ce RC with kl bound} & \multicolumn{2}{l|}{ce RC with $\lambda$ bound} \\ \midrule
Method   & Dataset             & Model & Train ce     & Test ce    & KL/n      & kl inverse          & asympt             & kl inverse             & asympt                 \\ \midrule
MFVI     & Binary Half         & 1L    & 0.0256       & 0.0281     & 0.0106    & \textbf{0.0703}     & 0.0581             & 0.0934                 & 0.0756                 \\
Gibbs p. & Binary Half         & 1L    & 0.0166       & 0.0166     & 0.0205    & 0.0706              & \textbf{0.0511}    & \textbf{0.0915}        & \textbf{0.0663}        \\
MFVI     & Binary              & 1L    & 0.0270       & 0.0272     & 0.0105    & \textbf{0.0707}     & 0.0580             & 0.0941                 & 0.0756                 \\
Gibbs p. & Binary              & 1L    & 0.0122       & 0.0125     & 0.0195    & 0.0598              & \textbf{0.0315}    & \textbf{0.0777}        & \textbf{0.0402}        \\ \midrule
MFVI     & $14 \times 14$ Half & 2L    & 0.0481       & 0.0481     & 0.0148    & \textbf{0.1238}     & 0.0947             & \textbf{0.1710}        & 0.1263                 \\
Gibbs p. & $14 \times 14$ Half & 2L    & 0.0335       & 0.0361     & 0.0477    & 0.1410              & \textbf{0.0946}    & 0.1888                 & \textbf{0.1237}        \\
MFVI     & $14 \times 14$      & 2L    & 0.0463       & 0.0460     & 0.0140    & 0.1196              & 0.0906             & 0.1631                 & 0.1194                 \\
Gibbs p. & $14 \times 14$      & 2L    & 0.0246       & 0.0259     & 0.0381    & \textbf{0.1118}     & \textbf{0.0702}    & \textbf{0.1484}        & \textbf{0.0910}        \\ \midrule
MFVI     & MNIST Half          & 2L    & 0.0430       & 0.0437     & 0.0199    & \textbf{0.1176}     & 0.0966             & \textbf{0.1570}        & 0.1263                 \\
Gibbs p. & MNIST Half          & 2L    & 0.0324       & 0.0356     & 0.0428    & 0.1347              & \textbf{0.0935}    & 0.1792                 & \textbf{0.1223}        \\
MFVI     & MNIST               & 2L    & 0.0423       & 0.0419     & 0.0196    & \textbf{0.1010}     & 0.0947             & \textbf{0.1317}        & 0.1226                 \\
Gibbs p. & MNIST               & 2L    & 0.0233       & 0.0253     & 0.0334    & 0.1065              & \textbf{0.0673}    & 0.1401                 & \textbf{0.0872}        \\ \bottomrule
\end{tabular}}
\label{ce_rc_table_old}
\end{table}

==> method_fig.tex <==




\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,295); %set diagram left start at 0, and has height of 295

%Straight Lines [id:da9317482072165887] 
\draw    (60,61) -- (79.17,103.18) ;
\draw [shift={(80,105)}, rotate = 245.56] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1398712631894372] 
\draw    (174,127) -- (214.57,87.4) ;
\draw [shift={(216,86)}, rotate = 135.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp11484070020949677] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.48 ] (8,19) -- (124,19) -- (124,55) -- (8,55) -- cycle ;
%Straight Lines [id:da999224619146638] 
\draw    (488,98) -- (533,97.04) ;
\draw [shift={(535,97)}, rotate = 178.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6915037751864055] 
\draw  [fill={rgb, 255:red, 228; green, 145; blue, 155 }  ,fill opacity=1 ] (10,108) -- (170,108) -- (170,159) -- (10,159) -- cycle ;
%Shape: Rectangle [id:dp9880556246573828] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.36 ] (221.05,33) -- (483.8,33) -- (483.8,154) -- (221.05,154) -- cycle ;
%Shape: Rectangle [id:dp4022843834206794] 
\draw  [fill={rgb, 255:red, 221; green, 218; blue, 218 }  ,fill opacity=1 ] (539,73) -- (649,73) -- (649,126) -- (539,126) -- cycle ;
%Shape: Rectangle [id:dp24999912860438356] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (221.05,57.67) -- (483.8,57.67) -- (483.8,86.5) -- (221.05,86.5) -- cycle ;
%Shape: Rectangle [id:dp48142280258936376] 
\draw  [fill={rgb, 255:red, 228; green, 145; blue, 155 }  ,fill opacity=1 ] (221.05,86.5) -- (483.8,86.5) -- (483.8,115.33) -- (221.05,115.33) -- cycle ;

% Text Node
\draw (12,20.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,xscale=0.8,yscale=0.8]  {$ \begin{array}{l}
\text{sample } w\ \sim Q^{*}\\
\text{with HMC}
\end{array}$};
% Text Node
\draw (227.5,35.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,xscale=0.8,yscale=0.8]  {$\text{compute }\mathrm{KL}\left( Q^{*} ||P\right)\text{from } w\ \text{and} \ P\ \text{with TI}$};
% Text Node
\draw (218,118.73) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xscale=0.8,yscale=0.8]  {$ \begin{array}{l}
 \text{c) \ estimate} \ \log p( z) \ \text{with TI}\text{ using Eqn. \ref{ti_logz_eq}} \ \\
\text{d) \ compute KL using Prop. \ref{prop31}}
\end{array}$};
% Text Node
\draw (12,113.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,xscale=0.8,yscale=0.8]  {$ \begin{array}{l}
\text{estimate} \ \hat{L}_{S}\left( Q^{*}\right) \ \text{from} \ w\\
\text{using a high-prob. bound}
\end{array}$};
% Text Node
\draw (546,82) node [anchor=north west][inner sep=0.75pt]  [font=\small,xscale=0.8,yscale=0.8] [align=left] {Compute bound\\by adding terms};
% Text Node
\draw (224,60.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,xscale=0.8,yscale=0.8] [align=left] {

a) \ \text{sample } $w\ \sim Q^{*\beta }$
};
% Text Node
\draw (224,90) node [anchor=north west][inner sep=0.75pt]  [font=\small,xscale=0.8,yscale=0.8] [align=left] {
{\small 
 \text{b) \ estimate} \ $\hat{L}_{S}\left( Q^{*\beta }\right)$ \ \text{with high-prob. bound}
}};


\end{tikzpicture}

